Observations of large-scale solar flows

In this dissertation, several components of large-scale solar flows are studied observationally: solar equatorial Rossby waves (waves of radial vorticity), large-scale convection, and surface flows around active regions. Maps of horizontal flows are derived from photospheric observations by the Helioseismic and Magnetic Imager (HMI) aboard the Solar Dynamics Observatory (SDO) using two different techniques: granulation tracking and local helioseismology. First, the eigenfunctions of solar Rossby waves are measured from helioseismic ring-diagram flow maps with a correlation method and a spectral analysis. Down to $9$ Mm below the surface, the dependence of the radial vorticity with radius $r$ is consistent with $r^{m-1}$, for a given longitudinal wavenumber $m$. At the surface, the eigenfunctions are complex-valued. The real part decreases away from the equator and switches sign around $\pm 20-30^\circ$. The imaginary part is small, but nonzero, and may be due to wave attenuation. This may have implications for the transport of angular momentum in the latitudinal direction. Second, we revisit previous measurements of power spectra of longitudinal velocities near the solar surface, obtained from time-distance and ring-diagram helioseismology. Several issues in these past helioseismic analyses are identified and corrected. The corrections are not sufficient to remove the discrepancy between the measurements. I thus present new velocity power spectra from granulation tracking and ring-diagram helioseismology. The two new measurements are close to each other near the solar surface, and the corresponding kinetic energy decreases with increasing spatial scale.

==> cv.tex <==
\chapter*{Curriculum vitae\markboth{Curriculum vitae}{Curriculum vitae}}
\addcontentsline{toc}{chapter}{Curriculum vitae}

% activate for CV on a separate page
% \thispagestyle{empty}

{\bf\Large Personal data}\\
\\
\begin{tabular}{ll}
Full name & Bastian Severin Niklas Proxauf \\
Date of Birth & 13 May 1993 \\
Place of Birth & Freistadt, Austria \\
Nationality & Austrian \\
\end{tabular}
\\\\\\
{\bf\Large Education}\\
\\
{\bf\large PhD student}\\
\\
\begin{tabular}{ll}
Oct. 2016 -- Apr. 2020 & at the International Max Planck Research School for Solar \\
 & System Science and the University of G{\"o}ttingen \\
Thesis & \textit{Observations of large-scale solar flows} \\
Advisors & Prof. Dr. Laurent Gizon, Dr. Bj{\"o}rn L{\"o}ptien, \\
 & Prof. Dr. Andreas Tilgner \\
\end{tabular}
\\\\\\
{\bf\large M.Sc. in Astrophysics}\\
\\
\begin{tabular}{ll}
Oct. 2014 -- Sep. 2016 & AstroMundus -- Erasmus Mundus Joint Master Program \\
 & in Astrophysics at the University of Innsbruck, the University of \\
 & Rome Tor Vergata, and the University of G{\"o}ttingen \\
Thesis & \textit{Homogeneous Metallicity Scale for Galactic Classical Cepheids} \\
Advisor & Prof. Dr. Giuseppe Bono (University of Rome Tor Vergata) \\
\end{tabular}
\\\\\\
{\bf\large B.Sc. in Physics}\\
\\
\begin{tabular}{ll}
Oct. 2010 -- June 2013 & at the University of Innsbruck \\
Thesis & \textit{Upgrading diagnostic diagrams of forbidden line emission:} \\
& \textit{The influence of modern atomic data} \\
Advisor & Prof. Dr. Stefan Kimeswenger \\
\end{tabular}
\\\\\\

